Consistency and Certain Answers in Relational to RDF Data Exchange with Shape Constraints

We investigate the data exchange from relational databases to RDF graphs inspired by R2RML with the addition of target shape schemas. We study the problems of consistency i.e., checking that every source instance admits a solution, and certain query answering i.e., finding answers present in every solution. We identify the class of constructive relational to RDF data exchange that uses IRI constructors and full tgds (with no existential variables) in its source to target dependencies. We show that the consistency problem is coNP-complete. We introduce the notion of universal simulation solution that allows to compute certain query answers to any class of queries that is robust under simulation. One such class are nested regular expressions (NREs) that are forward i.e., do not use the inverse operation. Using universal simulation solution renders tractable the computation of certain answers to forward NREs (data-complexity). Finally, we present a number of results that show that relaxing the restrictions of the proposed framework leads to an increase in complexity.

==> intro.tex <==
\section{Introduction}
\label{sec:introduction}
The recent decade has seen Resource Description Framework raise to the task of
interchanging data between Web applications~\cite{michel:2013}. In many
applications the data is stored in a relational database and only exported as
RDF, as evidenced by the proliferation of languages for mapping relational
database to RDF, such as R2RML, Direct Mapping or
YARRRML~\cite{yarrrml}. Although RDF has been originally proposed schema-less to
promote its adoption, the need for schema languages for RDF has been since
identified~\cite{w3c:2013, gayo:17}. For instance, one of the benefits of
working with data conforming to a schema is an increased execution safety: data
is validated against a schema prior to feeding it into applications which need
not to worry about handling malformed or invalid data that could otherwise cause
undesirable and difficult to predict side-effects. One family of proposed schema
formalisms for RDF is based on \emph{shape constraints} and this class includes
\emph{shape expressions schemas} (ShEx)
\cite{shexspec,staworko:2015a,boneva:hal-01590350} and \emph{shape constraint
  language} (SHACL) \cite{shaclspec,shacl-rec}. The two languages allow to
define a set of types that impose structural constraints on nodes and their
immediate neighborhood in an RDF graph. The following is an example of shape
constraints for RDF storing a collection of bug reports (here, $\col$ is a
default prefix):
\begin{align*}
  \Bug \to{}& \{ \descr \dbl \LitSym^\ONE, \rep \dbl \User^\ONE, \rel \dbl \Bug^\MANY\}\\
  \User \to{}& \{ \name\dbl \LitSym^\ONE, \mel\dbl \LitSym^\ONE,  \tracks\dbl \Bug^\PLUS\}%\\\prep\dbl \Test^\MAYBE,
\end{align*}
Essentially, the schema requires that each bug report has a description, a user
that reported it, and a number of related bug reports. Each user needs to a
name, an email, and has to track at least one bug report.

\emph{Data exchange} is the formal study of the process of taking data from a
\emph{source} database and transforming it into a \emph{target} instance, also
called a \emph{solution}. This process is defined with a set of
\emph{source-to-target dependencies} (std's) of the form
$\varphi\rightarrow\psi$, where $\varphi$ is a query over the source database
whose answers are used by $\psi$ to assert facts over the target
instance. Several problems of interest are studied. The very immediate problem
is constructing a solution. However, it is possible that for a given source
instance a solution may not exists if it is not possible to satisfy both the
std's and the target schema. Consequently, the problem of \emph{consistency} is
often studied: identifying data exchange settings that guarantee the existence
of a solution for any source instance. In general, there might be (infinitely)
many possible solutions and it is a standard practice to represent them all with
a \emph{universal solution}. In the presence of many solutions, queries are
interpreted under the possible worlds semantics~\cite{Lipski81}, giving raise to
\emph{certain answers} i.e., answers that are present in every
solution~\cite{fagin:2005a}. Interestingly, an important connection between
universal solutions and certain answers has been identified: certain answers to
a (positive) conjunctive query can be obtained by evaluating the query over the
universal solution.
  

In the present paper we consider the framework of relational to RDF data
exchange with target shape constraints and study the problems of checking
consistency and computing certain query answers using universal solutions. We
identify the class of \emph{constructive relational to RDF data exchange
  settings}, that consists of std's that use IRI constructors to explicitly
specify how to construct the node identifiers in the target RDF. This framework
closely captures the expressive power of Direct Mappings, an important subclass
of R2RML, that has been found to address many practical use
cases~\cite{medeiros:2015,SEQUEDA201319}. Additionally, our framework allows to
specify shape constraints on the target instance and allows the std's to specify
the types of the constructed RDF nodes.

Our first contribution is an algorithm for checking the consistency of
constructive data exchange settings. In \cite{boneva:18} we have considered the
same problem for a more restrictive case of fully-typed data exchange settings,
where all constructed RDF nodes need to be assigned a type. This requirement
allows to reduce the consistency problem to a simple test of propagating
functional dependencies (key constraints) from the relational source schema over
a view derived from the std's to a set of functional dependencies derived from
the target shape constraints. This technique can no longer be employed for
constructive data exchange setting, where the constructed RDF nodes need not be
typed, and to address it we propose a novel and non-trivial technique. We first
identify an exhaustive set of patterns in the target instance that capture
possible violation of the shape constraints. Next, by backtracking type
propagation and stds we identify patterns in a source instance (tableaux) that
could lead to an inconsistent target instance. Then, we attempt to find a
pattern that is consistent with the constraints of the source relational
schema. If such a tableaux is found, there exists a consistent source instance,
for which no solution satisfies the target shape constraints. Finally, we show
that checking consistency of constructive data exchange settings is
coNP-complete.

The second problem we study, and which we have not considered in our previous
work, is computing certain query answers. If the target RDF graph is viewed as a
relational structure, our framework is a special case of the standard relational
data exchange setting with guarded tuple-generating dependencies and we can use
the method proposed in~\cite{CALI201257} Cal\`{i} et al. to compute certain
answers to conjunctive queries (CQ). This method for a given bound $k$
constructs a solution that allows to compute certain answers to any conjunctive
query whose size is bounded by $k$. However, the constructed solution has size
exponential in $k$ and is not universal. In fact, it is known that a finite
universal solution need not exists even if we restrict our attention to
fully-typed relational to RDF data exchange~\cite{boneva:18}. More importantly,
the bound $k$ directly constraints the lengths of the paths that can be
inspected by a conjunctive query, and therefore, the above method cannot be
adapted to more general path queries that are highly relevant for querying graph
databases. To fill this gap we consider the class of \emph{nested regular
  expressions} (NREs) that have been proposed as the navigational core of a
popular RDF query language SPARQL~\cite{PEREZ2010255}. We identify its subclass
of \emph{forward NREs} that do not use the inverse axis, and which captures
regular path queries (RPQs), their unions, and their acyclic
conjunctions. Because of the lack of inverse, forward NREs are incomparable with
CQs and arbitrary conjunctions of RPQs. Interestingly, for forward NREs the
notion of universal solution can be weakened, to what we call \emph{universal
  simulation solution}, by replacing the use of homomorphisms with the standard
notion of graph simulation. It nevertheless allows to compute certain answers to
forward NREs. More importantly, the size of the universal simulation solution is
$O(n^2+2^{cm})$, where $n$ is the size of the source instance and $m$ is the
number of types used in the shape constraints and we prove that the exponential
bound is in fact tight.

% \noindent
% \textbf{TODO:} By comparing our framework with previous work give a light
% outline of the contents of this paper and our contributions.

% The contributions are summarized below.
% \begin{itemize}
% \item We present an algorithm for deciding the consistency of a constructive
%   data exchange setting.
% \item We propose the notion of a universal simulation solution, we identify
%   weakly recursive shape constraints that guarantee the existence of universal
%   simulation solutions, and we present a tractable construction of universal
%   simulation solutions.
% \item We study certain query answering. We identify the class of regular acyclic
%   patterns, a subclass of nested regular expressions without the inverse, and
%   show that universal simulation solutions are suitable for finding certain
%   answers to RAP. We also study certain answers to conjunctive queries using
%   existing results.
% \end{itemize}
 
% The Resource Description Framework (RDF) has become the de-facto standard for
% exchanging data on the Web \cite{Bizer:2011}. Often, the data is stored
% in a relational database and is exported in RDF format to be consumed by other
% applications using existing query techniques. A smooth interoperability between
% publishing and consuming applications is enabled by data that follows a prescribed
% structure, which is typically captured with a schema. Shape Expressions
% (ShEx)~\cite{staworko:2015a, boneva:hal-01590350} is one of the languages that have
% been proposed and it allows to define a set of \emph{types} that impose
% structural \emph{constraints} on nodes and their immediate \emph{neighborhood}
% in an RDF graph.

% % Shape Expressions (ShEx) \cite{staworko:2015a, boneva:hal-01590350} and SHACL
% % \cite{w3c:shacl} are two such languages and they both allow to define a set of
% % \emph{types} that impose structural \emph{constraints} on nodes of an RDF graph
% % and their immediate \emph{neighborhood}. (In this paper we focus on a fragment
% % of ShEx and discuss in Section~\ref{sec:discussion} how our results can be
% % transferred to SHACL.)
% % In the present paper we are interested in a subset of ShEx called DetShEx$_0$
% % implemented in ShEx 1.0 \cite{shex1}; we discuss

% Data exchange from relational databases to RDF in the presence of ShEx is the
% process of transforming an instance of a relational schema to an RDF graph,
% called a \emph{solution}, that satisfies a ShEx schema. This process is defined
% in a declarative fashion using a set of rules, called \emph{source-to-target
%   tuple generating dependencies} (st-tgds). There might be (possibly infinitely)
% many solutions and it is a standard practice to attempt to represent all of them
% using a \emph{universal solution}. In the presence of many solutions, queries
% are interpreted under the possible worlds semantics~\cite{Lipski81}, giving
% raise to \emph{certain answers} i.e., answers that are present in every
% solution~\cite{fagin:2005a}. Interestingly, certain answers to a (conjunctive)
% query can be obtained by evaluating the query over the universal solution.

% \begin{example}\label{ex:data-exchange}
%   Consider the relational database of bug reports in Figure~\ref{fig:db}. The
%   relation $\RBug$ stores information about bugs including description and the
%   user who reported it.  Users have a name (relation $\RUser$) and an email
%   (relation $\REmail$).  The relation $\RTrack$ stores which users track which
%   bugs, and tuples in the relation $\RRel$ indicate that a bug is related to
%   another bug.
% %	\vspace{-10pt}
% 	\begin{figure}[htb]
% 		\centering
% 		\vspace{-1em}		
% 	\begin{tabular}[t]{cc}
% 		\multicolumn{2}{c}{\RUser}\\
% 		\uline{\textit{uid}}& \textit{name}  \\[2pt]
% 		\hline
% 		1 & Jose \\
% 		2 & Edith89 \\
% 	\end{tabular}
% 	\hfill
% 	\begin{tabular}[t]{cc}
% 		\multicolumn{2}{c}{\REmail}\\
% 		\uline{\textit{uid}}& \textit{email} \\[2pt]
% 		\hline
% 		1 & j@ex.com
% 	\end{tabular}
% 	\hfill
% 	\begin{tabular}[t]{ccc}
% 		\multicolumn{2}{c}{\RTrack}\\
% 		\uline{\textit{uid}}& \uline{\textit{bid}}\\[2pt]
% 		\hline
% 		1 &  1\\ 
% 		1 &  2
% 	\end{tabular}
% 	\hfill
% 	\begin{tabular}[t]{ccc}
% 		\multicolumn{3}{c}{\RBug}\\
% 		\uline{\textit{bid}}& \textit{descr} & \textit{uid}\\[2pt]
% 		\hline
% 		1 & Boom! & 1 \\
% 		2 & Kabang! & 1 \\
% 		3 & Bang! & 2 
% 	\end{tabular}
% 	\hfill
% 	%		\\
% 	\begin{tabular}[t]{cc}
% 		\multicolumn{2}{c}{\RRel}\\
% 		\uline{\textit{bid}}& \uline{\textit{rid}} \\[2pt]
% 		\hline
% 		2 & 1 \\
% 		1 & 3
% 	\end{tabular}
% 		\caption{Relational source database\label{fig:db}}
% 	\end{figure}
% 	%	\vspace{-10pt}

%    \noindent
%    Now, suppose that we wish to export the above data to a partner application
%    that has an already existing infrastructure for consuming bug reports in the
%    form of an RDF graph whose structure follows this ShEx schema (where $\col$
%    is a default prefix):
% 	\begin{align*}
% 	\Bug \to{}& \{ \descr \dbl \LitSym^\ONE, \rep \dbl \User^\ONE, \rel \dbl \Bug^\MANY\}\\
% 	\User \to{}& \{ \name\dbl \LitSym^\ONE, \mel\dbl \LitSym^\ONE,  \tracks\dbl \Bug^\PLUS\}%\\\prep\dbl \Test^\MAYBE,
% 	\end{align*}
%    This schema states that a bug report must have a description, a user who
%    reported it, and possibly a number of related bug reports (cardinality
%    $\MANY$). A user has a name and an email address and tracks at least one bug
%    (cardinality $\PLUS$).  Figure~\ref{fig:rdf} presents an RDF graph that
%    satisfies the specified structure and captures the information in the
%    relational database. We point out that the graph uses a (labeled) null
%    literal $\bot_1$ for the email of Edith89 that is required by the ShEx schema
%    but is missing in the source database. It also contains a blank node
%    $\mathsf{\_\col{}b}$ to represent the required bug tracked by user
%    $\mathsf{anon\col{}2}$, and a blank node $\mathsf{\_\col{}u}$ to represent
%    the required user that reported the bug $\mathsf{\_\col{}b}$ (it does not
%    need to be the same as $\mathsf{anon\col{}2}$). The blank nodes
%    $\mathsf{\_\col{}b}$ and $\mathsf{\_\col{}u}$ have edges for the properties
%    required by their types \Bug and \User resp., and the values of these
%    properties are also nulls.
% \begin{figure}[htb]
% 	\centering 
% 	\vspace{-1em}
% 	\newcommand{\sequal}{\hspace{1pt}\mathord{=}\hspace{1pt}}
% 	\begin{tikzpicture}[>=latex]  

% \node (d3) at (-4,2.3) { ``Kabang!''};
% \node (d1) at (-1.5,2.5) { ``Boom!''};
% \node (d4) at (1.15,2.5) { ``Bang!''};
% \node (d2) at (4,2.5) {$\bot_4$};

% \node (bug3) at (-4,1) {$\mathsf{bug\col 2}$};
% \node (bug1) at (-1.5,1.25) {$\mathsf{bug\col 1}$};
% \node (bug4) at (1.15,1) {$\mathsf{bug\col 3}$};
% \node (bug2) at (4,1.25) {$\_\col \mathsf{b}$};

% \node (user1) at (-2.5,0) {$\mathsf{emp}\col\mathsf{jose}$};

% \node (user2) at (3.75,0) {$\_\col \mathsf{u}$};

% \node (emp1) at (0.9,-0.15) {$\mathsf{anon\col 2}$};  

% \node (n1) at (-3.5,-1.5) { ``Jose''};
% \node (e1) at (-1.75,-1.5) { ``j@ex.com''};

% \node (n2) at (4.7,-1.5) {$\bot_3$};
% \node (e2) at (3.1,-1.5) {$\bot_2$};
% \node (n3) at (0.1,-1.55) { ``Edith89''};
% \node (e3) at (1.5,-1.55) {$\bot_1$};

% \draw (user1) edge[->] node[above,sloped] {\name} (n1);
% \draw (user1) edge[->] node[above,sloped] {\mel} (e1);
% \draw (user1) edge[->,bend left=30] node[below,sloped] {\tracks} (bug3);
% \draw (user1) edge[->,bend right=50] node[below,sloped] {\tracks} (bug1);
% \draw (user2) edge[->] node[above,sloped] {\name} (n2);
% \draw (user2) edge[->] node[above,sloped] {\mel} (e2);
% \draw (user2) edge[->,bend right=70] node[below,sloped] {\tracks} (bug2);

% \draw (emp1) edge[->] node[above,sloped] {\name} (n3);
% \draw (emp1) edge[->] node[above,sloped] {\mel} (e3);
% \draw (emp1) edge[->,bend left=5] node[above,sloped] {\tracks} (bug2);
% \draw (bug1) edge[->] node[above,sloped] {\rel} (bug4);
% \draw (bug3) edge[->] node[above,sloped] {\rel} (bug1);
% \draw (bug1) edge[->] node[above,sloped] {\rep} (user1);
% \draw (bug1) edge[->] node[above,sloped] {\descr} (d1);

% \draw (bug2) edge[->] node[above,sloped] {\rep} (user2);
% \draw (bug2) edge[->] node[above,sloped] {\descr} (d2);

% \draw (bug3) edge[->] node[above,sloped] {\rep} (user1);
% \draw (bug3) edge[->] node[above,sloped] {\descr} (d3);

% \draw (bug4) edge[->] node[below,sloped] {\rep} (emp1);
% \draw (bug4) edge[->] node[above,sloped] {\descr} (d4);
% 	\end{tikzpicture}
% 	\caption{Target RDF graph (solution)\label{fig:rdf}}
% \end{figure}

% \noindent
% The transformation task is specified with the following set of logical rules
% (the free variables are implicitly universally quantified).
% 	\begin{align*}
% 		\RBug(b,d,u) \Rightarrow{}& \Triple(\bToI(b),\descr,d) \land \Bug(\bToI(b)) \land{}  \\
% 		&\Triple(\bToI(b),\rep,\pToI(u))\\
% \RRel(b_1,b_2) \Rightarrow{}& \Triple(\bToI(b_1),\rel,\bToI(b_2))\\
% 		\RUser(u,n) \Rightarrow{}& \Triple(\pToI(u),\name,n)\\% \land \User(\pToI(u)) \\
% 		 \RUser(u,n) \land \RTrack(u,b)  \Rightarrow{} 
% 		 &\Triple(\pToI(u),\tracks,\bToI(b))\\
% 		\RUser(u,n) \land \REmail (u,e) \Rightarrow{}& \Triple(\pToI(u), \mel, e)	
% 	\end{align*}
%    On the left-hand-side of each rule we employ queries over the source
%    relational database, while on the right-hand-side we make corresponding
%    assertions about the triples in the target RDF graph and the types of its
%    nodes.  The RDF graph from Figure~\ref{fig:rdf} is a possible solution of the
%    above source instance to this data exchange setting.  The values used in
%    relational tables are converted to valid RDF nodes with the help of the IRI
%    constructors $\pToI$ and $\bToI$ whose operation might be quite
%    sophisticated, and in particular, they may have the access to the source
%    database as well as other databases. For instance, the IRI constructor
%    $\pToI$ identified the user with id 1 as an employee Jose and assigned him
%    his corresponding IRI with the appropriate prefix $\mathsf{emp}$. On the
%    other had the user Edith89 is otherwise unknown to the application and was
%    assigned a fresh IRI with the prefix $\mathsf{anon}$. \qed
% \end{example}

% In the present paper we study two classical problems related to data exchange:
% \emph{consistency checking}, verifying that every valid source instance admits
% a solution, and computing \emph{certain answers}, answers that are present in
% every solution. We perform our study for a class of \emph{plain relational to
%   RDF data exchange settings}. This class allows to use the subclass of deterministic
% shape expressions schemas (DetShEx$_0$), which is known to be suitable to many
% practical applications~\cite{shex1} (in Section~\ref{sec:prelim} we briefly discuss
% how our results can be transferred to another schema language
% SHACL~\cite{w3c:shacl}). Because it is beyond the scope of this paper to analyze
% the precise operation of IRI constructors, we assume that the constructors are
% injective and their ranges are pairwise disjoint. Also, we only consider key
% dependencies in the source schema; foreign key constraints do not bring any
% useful information and can be in fact ignored.  The proposed framework allows
% only \emph{full} st-tgds, which do not permit existentially quantified variables
% on their right-hand side. This work is a follow-up to a previous
% paper~\cite{boneva:18} that studied consistency checking for a framework that
% additionally required the st-tgds to be fully typed i.e., every node in the
% triples on the right-hand side must have an explicitly specified ShEx type. In
% this paper we drop this requirement, which makes it a non-trivial extension and
% requires using novel techniques. We also point out that certain query
% answering has not been studied in~\cite{boneva:18}.

% % but because checking consistency involves
% % reasoning about st-tgds that generate edges for the same IRI, .

% The first contribution of the paper is an algorithm for deciding the consistency
% for plain data exchange settings. A data exchange setting is inconsistent if
% there exists a valid source instance that does not admit a target RDF graph that
% satisfies the ShEx schema. In general, ShEx schema is not satisfied by an RDF
% graph if there are missing edges (cardinalities \ONE and \PLUS) or if there are
% too many edges (cardinalities \ONE and \MAYBE). The former is not a concern in
% data exchange as we can always add additional blank nodes and edges to the
% solution. Consequently, the main reason for inconsistency springs up from ShEx
% constraints that bound the number of permitted outgoing edges (\ONE and
% \MAYBE). For instance, in Example~\ref{ex:data-exchange} a \User-node must have
% exactly one \mel. Since the \mel edges come only from the \REmail table and
% user id is its key, at most one \mel is provided for every user and if it is
% missing in the database a null value is used in the RDF graph. However, suppose
% that the source schema allows storing multiple emails per user, for instance, by
% extending the key constraint of \REmail to include also the \textit{email}
% attribute. Then, such setting would not be consistent because any source
%  instance containing a user with more than one email address would not
% admit a solution (that satisfies the ShEx schema). We also point out that the
% st-tgds do not specify explicitly that \mel edges are outgoing from \User-nodes
% but rather this information needs to be inferred, which introduces an
% additional degree of difficulty to the problem.

% Our approach addresses the challenge of consistency checking by combining two
% key ideas, which although technically very involved can be summarized as
% follows. We first identify an exhaustive set of patterns in the target RDF graph
% that capture possible violations of the ShEx schema. Then, by backtracking ShEx
% type propagation and the st-tgds, we identify a set of patterns in source
% instances that yield the RDF instances in question. Finally, we check if there
% is a source instance pattern that admits a source instance that satisfies all
% key dependencies. If this is the case, then there exists a source instance that
% does not admit a solution and the data exchange setting is not consistent;
% otherwise, it is consistent.

% % The presence of a target ShEx schema raises the problem of consistency of a data
% % exchange setting, i.e. whether all valid source instances admit a solution.  The
% % sole possible reason for inconsistency resides in the ShEx constraints that
% % impose maximal cardinality of some properties, for instance, a \Bug-node must
% % have exactly one \descr{}iption, a \User-node must have exactly one \mel.  We
% % can show that the data exchange setting from Example~\ref{ex:data-exchange} is
% % consistent.  It however wouldn't be the case if the source schema allowed
% % multiple e-mail addresses for the same user.  The latter is not immediate to
% % see, as the st-tgds defining the data-exchange setting do not even mention the
% % ShEx type \User, so one might think that the constraints regarding \User are
% % irrelevant.  A more careful look on the st-tgds reveals however that a \Bug-node
% % always has a \rep property, and from the ShEx schema we know that the value of
% % every \Bug's \rep property must be of type \User.  Consequently, there exist
% % source instances which solutions would contain \User nodes.  Nonetheless, this
% % alone is not a reason for inconsistency.  As is usual in data exchange, null
% % values do not allow to violate unicity constraints, as they can be replaced by
% % other null values or by constants.  A \User-node would violate the constraint of
% % unique \mel only if it has at least two \mel edges which values are different
% % \emph{constants}.  In order to show consistency of a data exchange setting, we
% % need to show that all ShEx types that could possibly appear in the solutions of
% % source instances (e.g. \User) and that define a property with a maximal allowed
% % number of occurrences (e.g. \mel) won't be associated to nodes in the solution
% % which properties contain a violation of the maximal cardinality.

% % Our first contribution is an algorithm for deciding the consistency of a data exchange setting under a reasonable restriction of the allowed IRI constructors, namely that they define injective functions with pairwise disjoint ranges.
% % We achieve this by identifying a finite number of patterns in the source instance that can lead to inconsistency.
% % If none of these patterns is compatible with the source key constraints, then the data exchange setting is consistent.
% % Each pattern is identified by ShEx type (eg \User), a property with maximal cardinality for this type (eg \mel), and an IRI constructor that can generate a node of this type (eg \pToI in the example).

% % \mycomment{TODO: point out that the schema in the example is recursive}
% % \mycomment{TODO: say that source instances have key constraints}

% Another important problem in data exchange is certain query answering. Certain
% answers to a query against the target schema are the answers that are present in
% every solution.  It is well known that, in the case of relational data exchange,
% a universal solution allows to compute the certain query answers to conjunctive
% queries (CQs) and even their unions~\cite{fagin:2005a}. In general, solutions
% that do not allow to compute certain answers are not desirable as they do not
% represent the source data faithfully. Unfortunately, a plain data exchange
% setting might admit only infinite universal solutions, even if it is
% consistent. For instance, a universal solution for the source instance and data
% exchange setting from Example~\ref{ex:data-exchange} is infinite, and contains
% an infinite path, required by the recursion between the \User and \Bug types:
% any bug is reported by a user, and any user tracks at least one bug.

% In general, whether or not a solution allows to compute the certain query
% answers depends on the kind of query. For RDF, important query languages are CQs
% and \emph{regular path queries} (RPQ), as well as the combination of both, known
% as conjunctive RPQs. As our second contribution, we propose a family of
% \emph{regular acyclic patterns} (RAP), which extend RPQs with nesting, and are
% precisely the subclass of nested regular expressions (NRE) without inverse. NREs
% have been proposed as a navigational core of SPARQL~\cite{PEREZ2010255}. For
% instance,
% %the following pattern 
% the RAP
% $ [\descr\cdot\langle\mathrm{Kabang!}\rangle]\cdot (\rel\cdot
% [\rep\cdot\name\cdot\langle\mathrm{Jose}\rangle])^*\cdot
% \rep\cdot\name\cdot\langle\mathrm{Edith89}\rangle $ tests whether there exists a
% bug with description ``Kabang'' that is related to a bug reported by Edith89
% through a chain of bugs reported by Jose. We point out that the above query
% cannot be expressed with RPQs or their Boolean combinations.

% While the standard universal solutions, suitable for computing certain answers
% to CQs, are defined using homomorphisms, we show that for RAPs it is sufficient
% to use the notion of graph simulation to define \emph{universal simulation
%   solutions}. We show that for consistent plain data exchange settings, a finite
% universal simulation solution always exists and a minimal one can be computed in
% time polynomial in the size of the source instance. For instance, in
% Example~\ref{ex:data-exchange} the solution in Figure~\ref{fig:rdf} is in fact a
% universal simulation solution obtained by representing the infinite \User and
% \Bug path with a simple loop. This gives a tractable method for computing
% certain answers to RAPs. We also show that existing results on relational data
% exchange with guarded tgds can be used to compute in PTIME certain answers to
% CQs. We point out, however, that the two results are orthogonal as RAPs and CQ
% are incomparable, and the techniques used are different. It remains an open question
% whether it is possible to combine the two approaches.



% % For given source instance $\Inst$, data exchange setting $\DES$ and target query
% % $q$, the certain answers of $q$ for $\Inst$ and $\DES$ are the answers to the
% % query $q$ that are common to all solutions of $\Inst$ to $\DES$.
% %
% % Naturally, 
 
% % As a second contribution we define a family of \emph{acyclic pattern queries} which are basically RPQs combined by the conjunction and union operator, and that have acyclic query graphs.
% % For example, Figure~\ref{fig:rap} shows a  Boolean acyclic pattern query that tests whether there exists a bug that is reproduced by Jose and is transitively \rel to bug4.

% % A second contribution of the paper is that certain query answering acyclic pattern queries is decidable for relational to RDF data exchange.
% % This is shown by introducing a \emph{universal simulation solution}.
% % This is a solution to a data exchange problem that, intuitively, allows to simulate all paths that are common to all the solutions.
% % We then show that [TODO].
 
% % \begin{figure}[htb]
% % 	\begin{tikzpicture}[sibling distance=60pt,level distance=3cm,edge from parent path={(\tikzparentnode) -- (\tikzchildnode)},node distance=2.5cm]
% % 	\begin{scope}[xshift=1cm,yshift=0cm]
% % 	\Tree [.\node(r){};	
% % 	\edge node[above,sloped] {$\rel\cdot\rel^*$};[.\node(n1){$\langle \mathsf{bug\col 3} \rangle$}; ]
% % 	\edge node[above,sloped] {$\rep\cdot \name$};
% % 	[.\node(n2){$\langle$Jose$\rangle $};]
% % 	]
% % 	\end{scope}
% % 	\begin{scope}[xshift=4cm,yshift=-3cm]
% % 	\node (bug1) at (5,3) {$\mathsf{bug\col 2}$};
% % 	\node[below left of=bug1] (bug2) {$\mathsf{bug\col 1}$};
% % 	\node[below of=bug2] (bug3) {$\mathsf{bug\col 3}$};
% % 	\node[below right of=bug1] (user1) {$\mathsf{emp}\col\mathsf{jose}$};
% % 	\node[below of=user1] (t1) {``Jose''};
% % 	\draw (bug1) edge[->] node[above,sloped] {\rel} (bug2);
% % 	\draw (bug2) edge[->] node[above,sloped] {\rel} (bug3);
% % 	\draw (bug1) edge[->] node[above,sloped] {\rep} (user1);
% % 	\draw (user1) edge[->] node[above,sloped] {\name} (t1);
% % 	\path (r) edge[dashed,->] (bug1);
% % 	\path (n1) edge[dashed,->] (bug3);
% % 	\path (n2) edge[dashed,->] (t1);
% % 	\end{scope}
% % 	\end{tikzpicture}
% % 	\caption{Regular Acyclic Pattern Query satisfied by graph in Figure \ref{fig:rdf}}\label{fig:rap}
% % \end{figure}
	

% \input{related}
% \medskip
% \noindent
\paragraph{Organization} In Section~\ref{sec:prelim} we present basic
notions. In Section~\ref{sec:data-exchange} we formalize relational to RDF data
exchange. In Section \ref{sec:consistency-des} we study the problem of
consistency. And finally, in Section~\ref{sec:query-answering} we study the
problem of certain query answering. Conclusions are in
Section~\ref{sec:concl-future-work}.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:
